Cognitive Radio Networks: Realistic or Not?

A large volume of research has been conducted in the cognitive radio (CR) area the last decade. However, the deployment of a commercial CR network is yet to emerge. A large portion of the existing literature does not build on real world scenarios, hence, neglecting various important interactions of the research with commercial telecommunication networks. For instance, a lot of attention has been paid to spectrum sensing as the front line functionality that needs to be completed in an efficient and accurate manner to enable an opportunistic CR network architecture. This is necessary to detect the existence of spectrum holes without which no other procedure can be fulfilled. However, simply sensing (cooperatively or not) the energy received from a primary transmitter cannot enable correct dynamic spectrum access. For example, the low strength of a primary transmitter's signal does not assure that there will be no interference to a nearby primary receiver. In addition, the presence of a primary transmitter's signal does not mean that CR network users cannot access the spectrum since there might not be any primary receiver in the vicinity. Despite the existing elegant and clever solutions to the DSA problem no robust, implementable scheme has emerged. In this paper, we challenge the basic premises of the proposed schemes. We further argue that addressing the technical challenges we face in deploying robust CR networks can only be achieved if we radically change the way we design their basic functionalities. In support of our argument, we present a set of real-world scenarios, inspired by realistic settings in commercial telecommunications networks, focusing on spectrum sensing as a basic and critical functionality in the deployment of CRs. We use these scenarios to show why existing DSA paradigms are not amenable to realistic deployment in complex wireless environments.

==> scope.tex <==
\section{Scope of our Work \& Conclusions}
\label{sec:scope} 
\setcounter{paragraph}{0}

In this challenge paper we have tried to shed some light on the reasons behind the lack of commercial deployment of a cognitive radio network. In order to do so we focused on a specific functionality, important for the operations of such a network, that of spectrum sensing.  
However, we would like to emphasize on the fact that similar problems exist with respect to other functionalities, such as spectrum sharing and spectrum access. We emphasize that our work should not be viewed only as a question about the realization of cognitive radio networks. It should be seen more broadly as a challenge to the real world applicability of a large volume of existing research. For example, the research community is used to putting aside, in the majority of the cases, solutions that require large scale infrastructural changes. Without trying to argue in this paper whether this is correct or not, sometimes the only feasible solution(s) is(are) accompanied by this ``drawback". Thus, we should be more open to them and less critical of similar proposals. After all this is often the way that the world of commercial network operators functions.  

To sum up, solutions to technical problems might be much easier than we think. Coming back to the topic of this paper, CR networks, the nature of the primary user and the actual operations of a real communication system are usually neglected or made complicated or oversimplified. Therefore, the solutions proposed do not drive an effective commercially viable network architecture.  
Drastic solutions often need to be taken, but for this, a careful examination of the ``real" underlying tradeoffs need to be considered. For instance, in our sketch solution, for eliminating broadcast TV completely, the involved parties need to consider the potential benefits from the capacity/revenues obtained by freeing up the spectrum as well as the cost to serve people through other technologies (potentially for free).  

\vspace{-0.1in}
